A time-adaptive finite element phase-field model suitable for rate-independent fracture mechanics

The modeling of cracks is an important topic - both in engineering as well as in mathematics. Since crack propagation is characterized by a free boundary value problem (the geometry of the crack is not known beforehand, but part of the solution), approximations of the underlying sharp-interface problem based on phase-field models are often considered. Focusing on a rate-independent setting, these models are defined by a unidirectional gradient-flow of an energy functional. Since this energy functional is non-convex, the evolution of the variables such as the displacement field and the phase-field variable might be discontinuous in time leading to so-called brutal crack growth. For this reason, solution concepts have to be carefully chosen in order to predict discontinuities that are physically reasonable. One such concept is that of Balanced Viscosity solutions (BV solutions). This concept predicts physically sound energy trajectories that do not jump across energy barriers. The paper deals with a time-adaptive finite element phase-field model for rate-independent fracture which converges to BV solutions. The model is motivated by constraining the pseudo-velocity of the crack tip. The resulting constrained minimization problem is solved by the augmented Lagrangian method. Numerical examples highlight the predictive capabilities of the model and furthermore show the efficiency and the robustness of the final algorithm.

==> Chap_AMnotBV_Fformulation.tex <==
\section{Example: Alternate minimization in general does not generate balanced viscosity solutions}

All the numerical experiments presented in Section~\ref{sec:Experiments} and also in \cite{boddin_approximation_2022} suggest that the pure AM scheme without the E\&M constraint converges to a BV solution as well. In order to show that this is not a general property of the scheme, an example with a structure similar to the damage model but with finite state spaces is given next. But first it will be shed light on the mathematical background of this works subject.

As explained in Section~\ref{sec:Theory}, we are looking for minimizers $z$ of the total energy functional $\calF(t,u,z)$ under irreversibility constraint $\dot{z}\leq 0$ a.e. in $\Omega$
 or equivalently for minimizers of
\begin{align}\label{eq:F+H}
	z\mapsto \calF(t,u,z)+\calH(\dot{z})
\end{align}
with the convex and positive 1-homogeneous functional $\calH$ given by
\begin{align*}
	\calH(\dot{z})\coloneqq \begin{cases}
		0,& \dot{z}\leq 0\text{ a.e. in }\Omega\\
		\infty,& \text{otherwise.}
	\end{cases}
\end{align*}
Due to the convexity of \eqref{eq:F+H}, minimizers $z$ are exactly the stationary points, i.e. $z$ with
\begin{align}\label{eq:stationarity}
	0\in \D_z\calF(t,u,z)+\partial\calH(\dot{z}),
\end{align}
where the derivative of $\calH$ in $v$ is given in terms of the set-valued subdifferential $\partial\calH(v)$. 

Likewise $\calF(t,u,z)$ should be minimized in $u$, which is due to convexity in $u$ equivalent to the balance of linear momentum
\begin{align}\label{eq:balanceoflinearmomentum}
	\D_u\calF(t,u,z)=0.
\end{align}
Thus we are looking for $u$ and $z$, that satisfy \eqref{eq:stationarity} as well as \eqref{eq:balanceoflinearmomentum}. Instead we could also consider the \textit{reduced problem}
\begin{align}\label{eq:reducedproblem}
	0\in\D_z\calF_{\text{red}}(t,z)+\partial\calH(\dot{z}),
\end{align}
with the \textit{reduced energy} $\calF_{\text{red}}(t,z)$ given by
\begin{align*}
	\calF_{\text{red}}(t,z)\coloneqq \calF(t,u_{\text{min}}(t,z),z),
\end{align*}
where $u_\text{min}(t,z)$ is the uniquely determined minimizer of $u\mapsto\calF(t,u,z)$ for given $t$ and $z$. However, within this paper $\calF_{\text{red}}$ is mainly used to facilitate the graphical visualization in Figures \ref{fig:localStability} and \ref{fig:reducedEnergy}. It is not used within the algorithmic schemes for the approximation of a solution. There $\calF(t,u,z)$ is alternately minimized in $u$ and $z$ for each time step $t$. 

But for the moment let us stick to $\calF_{\text{red}}$ to make some theoretical observations. Due to the positive 1-homogeneity of $\calH$, the subdifferential of $\calH$ at any point is included in the subdifferential of $\calH$ at $0$. Therefore we find the local stability 
\begin{align}\label{eq:localstability}
	0\in \D_z\calF_{\text{red}}(t,z)+\partial\calH(0)
\end{align}
as a necessary condition for \eqref{eq:reducedproblem}.
Notice that $\calF_{\text{red}}$ is not convex in $z$. In a system with a non convex energy functional -- as in our case -- a solution might necessarily has to evolve discontinuously in time to stay in the set of locally stable states
\begin{align}\label{eq:locallyStableStates}
	\left\{(t,z): 0\in\D_z\calF_{\text{red}}(t,z)+\partial \calH(0)\right\},
\end{align}
i.e. it develops jumps.
This can already be observed within simplified toy examples, cf. Figure~\ref{fig:localStability} -- in this picture the set of locally stable states \eqref{eq:locallyStableStates} corresponds to the gray area; starting at $t=0$ with an initial value in the (upper) gray area, e.g. $z_0=33.5$, as time evolves, a solution necessarily has to jump across the white area (where \eqref{eq:localstability} is not satisfied) to stay in the (lower) gray area for times lager than $t\approx 1.28$. Thus in the non convex case differential formulation \eqref{eq:reducedproblem} can not be used, since it includes the time derivative $\dot{z}(t)$ of a solution, which is not defined at times $t$ where the solution jumps. In this regard another advantage of the concept of \textit{global energetic solutions} is their derivative-free formulation. However, as mentioned in the introduction global energetic solutions are forced to leave a locally stable state, if it is not globally stable as well. In other words, they might jump across energy barriers and thus jumps occur earlier than physically expected. Therefore our focus lies on \textit{balanced viscosity (BV) solutions}, that stay as long as possible in the set of locally stable states and thus do not jump across energy barriers and behave physically reasonable. Their notion was derived by viscously regularizing differential inclusion \eqref{eq:reducedproblem} via
\begin{align}\label{eq:viscousregularization}
	0\in \D_z\calF_{\text{red}}(t,z)+\partial\calH(\dot{z})+ \epsilon\dot{z}
\end{align}
with a small viscosity parameter $\epsilon>0$ and passing for solutions $z_\epsilon$ of \eqref{eq:viscousregularization} to the limit $\epsilon\downarrow 0$ -- a \textit{vanishing viscosity approach}. This way the limiting solution, respectively the concept of BV solutions, comprises a finer description of the jumps. They are specified as viscous transition paths between two locally stable states.

%
\begin{figure}[http]
	\centering
	{\begin{psfrags}%
			\psfrag{z}[mc][tc][1][270]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large$z$\end{tabular}}%
			\psfrag{t}[tc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\Large$t$\end{tabular}}%
			\begin{tikzpicture}
				\node at (0,0) {\includegraphics[scale=0.7]{AMnotBV/stableSet.eps}};
				\node at (6,2) {\includegraphics[scale=0.6]{AMnotBV/stableSetZoom.eps}};
				\node (rect) at (1.15,3.77) [draw,black,thick,minimum width=2cm,minimum height=0.3cm] {};
				\draw[black,thick] (0.15,3.92)--(3.94,4.555);
				\draw[black,thick] (0.15,3.615)--(3.938,-0.24);
				\node (rect) at (8,-2.35) [draw,black,thick,minimum width=5cm,minimum height=2.7cm] {};
				\draw[red,line width=0.5mm] (6,-2.3)--(6.5,-2.3);
				\node at (8.2,-2.3) [black] {pure AM scheme};
				\draw[blue,line width=0.8mm,dash pattern=on 0.7mm off 0.7mm] (6,-1.6)--(6.5,-1.6);
				\node at (8.22,-1.6) [black] {combined scheme};
				\node (rect) at (6.25,-3) [draw,gray!75,fill=lightgray!60,minimum width=0.5cm,minimum height=0.5cm] {};
				\node at (8.41,-3) [black] {locally stable states};
			\end{tikzpicture}
	\end{psfrags}}
	\caption{Outcome of schemes for approximating solutions of the rate-independent system driven by energy and dissipation given in \eqref{eq:energy} and \eqref{eq:dissipation}: Set of locally stable states \eqref{eq:locallyStableStates} in the $(t,z)$-plane (gray area); the combined scheme (dashed blue) for $\rho=0.001$ and the pure alternate minimization scheme (red) with equidistant time steps $\Delta t=\rho$ both for initial value $z_0=33.5$ and with 20 alternate minimization iterations per time step.}\label{fig:localStability}
\end{figure}
%

With regard to the promised example, the energy
\begin{align}\notag
	\calF(t,u_1,u_2,z) \coloneqq 58(z+14)^2&+ u_1^2\left(60(z+2)^2+76\right)+u_1\left(-4(z-16)^2-8\right)\\
	&+u_2^2\left(15(z-33)^2+100\right)+25 u_2(z-20)^2\underbrace{-2000t u_2}_{\eqqcolon \ell(t,u_2)}\quad\text{for } t\geq 0, u_1,u_2,z\in\R \label{eq:energy}
\end{align}
structurally similar to the energy functional of the damage model considered in \cite{boddin_approximation_2022} and in this paper is chosen. Indeed, it is separately convex and even separately quadratic in the variables $u=(u_1,u_2)$ and $z$. An external loading in $u_2$ direction is included with the term $\ell(t,u_2)$. 

As above an \textit{irreversibility constraint} is guaranteed via the convex and positive 1-homogeneous functional $\calH$ given by
\begin{align}\label{eq:dissipation}
	\calH(\dot{z})\coloneqq
	\begin{cases}
		0, & \text{ for } \dot{z}\leq 0\\
		\infty, & \text{otherwise}.
	\end{cases}
\end{align}

Figure~\ref{fig:localStability} visualizes the outcome for $z$ of the combined scheme (dashed blue) and the pure alternate minimization scheme (red) applied to the energy and dissipation given in \eqref{eq:energy} and \eqref{eq:dissipation}. Moreover, utilizing the reduced energy $\calF_{\text{red}}$ it depicts the locally stable states (gray area), cf. \eqref{eq:locallyStableStates}. For the combined scheme arc-length parameter $\rho=0.001$ is chosen, whereas the pure alternate minimization scheme is realized with equidistant time steps $\Delta t=\rho$. Both schemes are initialized with $z_0=33.5$ and perform 20 alternate minimization iterations per time step.

It can be observed that both approximated solutions stay constant at the value $z=33.5$ up to time $t\approx 1.16$. Then they start to evolve continuously up to time $t\approx 1.28$, where both of them jump. But they jump into two differing states. The combined scheme produces a solution that jumps just as far as necessary to reach a locally stable state (gray area) again. Whereas the solution generated by the pure alternate minimization scheme jumps much further, in particular it jumps across some locally stable states. 

%
\begin{figure}[http]
	\centering
	\subcaptionbox{$t_{1}=0.001$\label{fig:redEner_Plots1}}
	{\begin{psfrags}%
			\psfrag{z}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$z$\end{tabular}}%
			\psfrag{Fred}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$\calF_{\text{red}}(t_1,z)$\end{tabular}}%
			\includegraphics[scale=0.35]{AMnotBV/Fk0.eps}
	\end{psfrags}}
	%\subcaptionbox{$\bar u(t_{93})=0.226\,\text{[mm]}$\label{fig:redEner_Plots2}}
	%{\includegraphics[scale=0.36]{k999.eps}}
	\subcaptionbox{$t_{1680}=1.27558$\label{fig:redEner_Plots3}}
	{\begin{psfrags}%
			\psfrag{z}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$z$\end{tabular}}%
			\psfrag{Fred}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$\calF_{\text{red}}(t_{1680},z)$\end{tabular}}%
			\includegraphics[scale=0.35]{AMnotBV/Fk1679.eps}
	\end{psfrags}}
	\subcaptionbox{$t_{1701}=1.27562$\label{fig:redEner_Plots4}}
	{\begin{psfrags}%
			\psfrag{z}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$z$\end{tabular}}%
			\psfrag{Fred}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$\calF_{\text{red}}(t_{1701},z)$\end{tabular}}%
			\includegraphics[scale=0.35]{AMnotBV/Fk1700.eps}
	\end{psfrags}}
	\\\vspace{10pt}
	\subcaptionbox{$t_{11001}=1.27562$\label{fig:redEner_Plots5}}
	{\begin{psfrags}%
			\psfrag{z}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$z$\end{tabular}}%
			\psfrag{Fred}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$\calF_{\text{red}}(t_{11001},z)$\end{tabular}}%
			\includegraphics[scale=0.35]{AMnotBV/Fk11000.eps}
	\end{psfrags}}
	%\subcaptionbox{$\bar u(t_{201})=0.226\,\text{[mm]}$\label{fig:redEner_Plots6}}
	%{\includegraphics[scale=0.16]{AMnotBV/k32000.eps}}
	\subcaptionbox{$t_{37124}=1.27562$\label{fig:redEner_Plots7}}
	{\begin{psfrags}%
			\psfrag{z}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$z$\end{tabular}}%
			\psfrag{Fred}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$\calF_{\text{red}}(t_{37124},z)$\end{tabular}}%
			\includegraphics[scale=0.35]{AMnotBV/Fk37123.eps}
	\end{psfrags}}
	\subcaptionbox{$t_{37849}=2.00052$\label{fig:redEner_Plots8}}
	{\begin{psfrags}%
			\psfrag{z}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$z$\end{tabular}}%
			\psfrag{Fred}[mc][tc][1]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}\small$\calF_{\text{red}}(t_{37849},z)$\end{tabular}}%
			\includegraphics[scale=0.35]{AMnotBV/Fk37848.eps}
	\end{psfrags}}
	\caption{Reduced energy $\calF_{\text{red}}(t,z)$ at several time steps $t$: Result of the time-adaptive scheme combined with alternate minimization (blue square) for $\rho=0.001$ and the pure alternate minimization scheme (red circle) with the same time steps as in the time-adaptive scheme each for initial value $z_0=33.5$ and with 20 alternate minimization iterations per time step.}\label{fig:reducedEnergy}
\end{figure}
%

To illustrate the types of minima (global/local) that are obtained at each time with the solutions generated by the two schemes, the reduced energy $z\mapsto\calF_{\text{red}}(t,z)$ is plotted at several time steps $t$ and its values at the corresponding states of the solutions generated by the combined scheme (blue square) and the pure alternate minimization scheme (red circle) are highlighted in Figure~\ref{fig:reducedEnergy}. For a better comparison of the two approximated solutions (especially to obtain common time steps), the alternate minimization scheme was performed again, but with the same time steps as for the time-adaptive scheme.

Figure~\ref{fig:redEner_Plots1}-\ref{fig:redEner_Plots3} exhibits that the generated solutions stay both in a locally but not globally stable state up to time $t\approx 1.28$ -- together with Figure~\ref{fig:localStability} it can even be inferred that the irreversibility constraint is active up to time $t\approx 1.16$ and that a local but not global minimum of $\calF_{\text{red}}$ is attained by the solutions between $t\approx 1.16$ and $t\approx 1.28$. Then at time $t\approx 1.28$ both solutions jump, cf. Figure~\ref{fig:redEner_Plots3}-\ref{fig:redEner_Plots7}. Within iterations $1701$ and $37124$, cf. Figure~\ref{fig:redEner_Plots4}-\ref{fig:redEner_Plots7}, the time is not incremented but stays fixed at $t\approx 1.28$. The constrained scheme generates the fine description of its solutions jump path to the next local minimum of $z\mapsto\calF_{\text{red}}(t,z)$ during these iterations. In contrast the solution produced by the pure alternate minimization scheme jumped mainly within iteration $1681$ and right into the global minimum of $z\mapsto\calF_{\text{red}}(t,z)$. As time further evolves both schemes stay in their respective local minimum, cf. Figure~\ref{fig:redEner_Plots8}.

It is noteworthy that the pure alternate minimization scheme, cf. Figure~\ref{fig:redEner_Plots1}-\ref{fig:redEner_Plots3} stayed at first in a locally but not globally stable state, i.e. it did not jump across an energy barrier. But in the further process it behaved conversely and jumped across an energy barrier into the globally stable state, cf. Figure~\ref{fig:redEner_Plots4}. Thus it does neither give a global energetic solution nor does it produce a balanced viscosity solution. Indeed, in the definition of BV solutions from \cite[Theorem~3.15]{boddin_approximation_2022} the balance of linear momentum has to be satisfied even along the jump path, such that jumps across energy barriers of the reduced energy $\calF_{\text{red}}$ contradict the claimed energy dissipation balance.




